On the Relationship Between Network Topology and Throughput in Mesh Optical Networks

The relationship between topology and network throughput of arbitrarily-connected mesh networks is studied. Taking into account nonlinear channel properties, it is shown that throughput decreases logarithmically with physical network size with minor dependence on network ellipticity.

==> tikz/dummy.tex <==
%
